Regularity of calibrated sub-actions for circle expanding maps and Sturmian optimization

In this short and elementary note, we study some ergodic optimization problems for circle expanding maps. We first make an observation that if a function is not far from being convex, then its calibrated sub-actions are closer to convex functions in certain effective way. As an application of this simple observation, for circle doubling map, we generalize a result of Bousch saying that translations of the cosine function are uniquely optimized by Sturmian measures. Our argument follows the mainline of Bousch's original proof, while the technical part is simplified by the observation mentioned above, and no numerical calculation is needed.

==> preamble.tex <==
%\pdfoutput=1
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{txfonts} % this changes mathcal
%\usepackage{amsfonts}
\usepackage{extarrows}
%\usepackage[colorlinks,linkcolor=blue]{hyperref}
\usepackage[colorlinks, linkcolor=blue]{hyperref}
%\usepackage[notref,notcite]{showkeys}
%\usepackage{stmaryrd}
%\usepackage{wasysym}

%\usepackage{ntheorem}

\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem*{thmA}{Theorem~A}
\newtheorem*{thmB}{Theorem~B}
\newtheorem{prop}[thm]{Proposition}
%\newtheorem{prop}{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{fact}[thm]{Fact}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{exe}{Exercise}[section]


\newtheorem*{clm}{Claim}
%\newtheorem*{lem}{Lemma}
%\newtheorem*{prop}{Proposition}

\theoremstyle{remark}
%\newtheorem*{clm}{Claim}
%\newtheorem*{exe}{Exercise}
\newtheorem*{rmk}{Remark}
\newtheorem*{exa}{Example}
\newtheorem*{ntn}{Notation}

\newcommand{\abs}[1] {\left|{#1}\right|}  %absolute value
\newcommand{\norm}[1] {\left\|{#1}\right\|} %norm
\newcommand{\brac}[1] {\left({#1}\right)}  %round brackets
\newcommand{\Brac}[1] {\left\{\,{#1}\,\right\}} %curly brackets
\newcommand{\floor}[1] {\left\lfloor\,{#1}\,\right\rfloor} %curly brackets
\newcommand{\ceil}[1] {\left\lceil\,{#1}\,\right\rceil}
%\newcommand{\pd}[2] {\dfrac{\partial {#1}}{\partial {#2}}} %first order partial derivative
\newcommand{\inp}[1]{\langle{#1}\rangle} %inner product
\newcommand{\pal} {\partial} %partial
\newcommand{\pd}[2] {\partial_{{#2}}{#1}} %first order partial derivative
\newcommand{\spd}[2] {\dfrac{\partial^2 {#1}}{\partial {#2}^2}} %second order partial derivative
\newcommand{\mspd}[3]{\dfrac{\partial^2 {#1}}{\partial {#2}\partial {#3}}} %second order mixed partial derivative

\newcommand{\sgn}{\mathrm{sgn}}
%%%%%%%%%%%%%%

% constants and notations to be determined

\newcommand{\ve}{\varepsilon}

\newcommand{\const}{\mathrm{Const}}


\newcommand{\eps}{\varepsilon}

\newcommand{\hrho}{\hat{\rho}}

\newcommand{\hxi}{\widehat{\xi}}

\newcommand{\hXi}{\hat{\Xi}}
\newcommand{\hzeta}{\hat{\zeta}}
\newcommand{\tzeta}{\tilde{\zeta}}

\newcommand{\homega}{\hat{\omega}}
\newcommand{\hdelta}{\hat{\delta}}

\newcommand{\hLambda}{\widehat{\Lambda}}

%\renewcommand{\le}{\leqslant}
%\renewcommand{\ge}{\geqslant}

\newcommand{\tmu}{\tilde{\mu}}
\newcommand{\teta}{\tilde{\eta}}
\newcommand{\tepsilon}{\tilde{\epsilon}}

\newcommand{\tomega}{\tilde{\omega}}

\newcommand{\mbba}{\mathbb{A}}
\newcommand{\mbbb}{\mathbb{B}}
\newcommand{\mbbc}{\mathbb{C}}
\newcommand{\mbbd}{\mathbb{D}}
\newcommand{\mbbe}{\mathbb{E}}
\newcommand{\mbbf}{\mathbb{F}}
\newcommand{\mbbg}{\mathbb{G}}
\newcommand{\mbbh}{\mathbb{H}}
\newcommand{\mbbi}{\mathbb{I}}
\newcommand{\mbbj}{\mathbb{J}}
\newcommand{\mbbk}{\mathbb{K}}
\newcommand{\mbbl}{\mathbb{L}}
\newcommand{\mbbm}{\mathbb{M}}
\newcommand{\mbbn}{\mathbb{N}}
\newcommand{\mbbo}{\mathbb{O}}
\newcommand{\mbbp}{\mathbb{P}}
\newcommand{\mbbq}{\mathbb{Q}}
\newcommand{\mbbr}{\mathbb{R}}
\newcommand{\mbbs}{\mathbb{S}}
\newcommand{\mbbt}{\mathbb{T}}
\newcommand{\mbbu}{\mathbb{U}}
\newcommand{\mbbv}{\mathbb{V}}
\newcommand{\mbbw}{\mathbb{W}}
\newcommand{\mbbx}{\mathbb{X}}
\newcommand{\mbby}{\mathbb{Y}}
\newcommand{\mbbz}{\mathbb{Z}}


\newcommand{\mbbnz}{\mathbb{N}_0}

\newcommand{\mbfa}{\mathbf{A}}
\newcommand{\mbfb}{\mathbf{B}}
\newcommand{\mbfc}{\mathbf{C}}
\newcommand{\mbfd}{\mathbf{D}}
\newcommand{\mbfe}{\mathbf{E}}
\newcommand{\mbff}{\mathbf{F}}
\newcommand{\mbfg}{\mathbf{G}}
\newcommand{\mbfh}{\mathbf{H}}
\newcommand{\mbfi}{\mathbf{I}}
\newcommand{\mbfj}{\mathbf{J}}
\newcommand{\mbfk}{\mathbf{K}}
\newcommand{\mbfl}{\mathbf{L}}
\newcommand{\mbfm}{\mathbf{M}}
\newcommand{\mbfn}{\mathbf{N}}
\newcommand{\mbfo}{\mathbf{O}}
\newcommand{\mbfp}{\mathbf{P}}
\newcommand{\mbfq}{\mathbf{Q}}
\newcommand{\mbfr}{\mathbf{R}}
\newcommand{\mbfs}{\mathbf{S}}
\newcommand{\mbft}{\mathbf{T}}
\newcommand{\mbfu}{\mathbf{U}}
\newcommand{\mbfv}{\mathbf{V}}
\newcommand{\mbfw}{\mathbf{W}}
\newcommand{\mbfx}{\mathbf{X}}
\newcommand{\mbfy}{\mathbf{Y}}
\newcommand{\mbfz}{\mathbf{Z}}


\newcommand{\mcla}{\mathcal{A}}
\newcommand{\mclb}{\mathcal{B}}
\newcommand{\mclc}{\mathcal{C}}
\newcommand{\mcld}{\mathcal{D}}
\newcommand{\mcle}{\mathcal{E}}
\newcommand{\mclf}{\mathcal{F}}
\newcommand{\mclg}{\mathcal{G}}
\newcommand{\mclh}{\mathcal{H}}
\newcommand{\mcli}{\mathcal{I}}
\newcommand{\mclj}{\mathcal{J}}
\newcommand{\mclk}{\mathcal{K}}
\newcommand{\mcll}{\mathcal{L}}
\newcommand{\mclm}{\mathcal{M}}
\newcommand{\mcln}{\mathcal{N}}
\newcommand{\mclo}{\mathcal{O}}
\newcommand{\mclp}{\mathcal{P}}
\newcommand{\mclq}{\mathcal{Q}}
\newcommand{\mclr}{\mathcal{R}}
\newcommand{\mcls}{\mathcal{S}}
\newcommand{\mclt}{\mathcal{T}}
\newcommand{\mclu}{\mathcal{U}}
\newcommand{\mclv}{\mathcal{V}}
\newcommand{\mclw}{\mathcal{W}}
\newcommand{\mclx}{\mathcal{X}}
\newcommand{\mcly}{\mathcal{Y}}
\newcommand{\mclz}{\mathcal{Z}}

\newcommand{\hmclt}{\hat{\mathcal{T}}}

\newcommand{\msca}{\mathscr{A}}
\newcommand{\mscb}{\mathscr{B}}
\newcommand{\mscc}{\mathscr{C}}
\newcommand{\mscd}{\mathscr{D}}
\newcommand{\msce}{\mathscr{E}}
\newcommand{\mscf}{\mathscr{F}}
\newcommand{\mscg}{\mathscr{G}}
\newcommand{\msch}{\mathscr{H}}
\newcommand{\msci}{\mathscr{I}}
\newcommand{\mscj}{\mathscr{J}}
\newcommand{\msck}{\mathscr{K}}
\newcommand{\mscl}{\mathscr{L}}
\newcommand{\mscm}{\mathscr{M}}
\newcommand{\mscn}{\mathscr{N}}
\newcommand{\msco}{\mathscr{O}}
\newcommand{\mscp}{\mathscr{P}}
\newcommand{\mscq}{\mathscr{Q}}
\newcommand{\mscr}{\mathscr{R}}
\newcommand{\mscs}{\mathscr{S}}
\newcommand{\msct}{\mathscr{T}}
\newcommand{\mscu}{\mathscr{U}}
\newcommand{\mscv}{\mathscr{V}}
\newcommand{\mscw}{\mathscr{W}}
\newcommand{\mscx}{\mathscr{X}}
\newcommand{\mscy}{\mathscr{Y}}
\newcommand{\mscz}{\mathscr{Z}}

\newcommand{\mfkc}{\mathfrak{C}}

\newcommand{\cB}{\check{B}}
\newcommand{\cD}{\check{D}}
\newcommand{\cI}{\check{I}}
\newcommand{\cJ}{\check{J}}


\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hc}{\hat{c}}
\newcommand{\hd}{\hat{d}}
\newcommand{\he}{\hat{e}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hg}{\hat{g}}
\newcommand{\hh}{\hat{h}}
\newcommand{\hi}{\hat{i}}
\newcommand{\hj}{\hat{j}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hl}{\hat{l}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hn}{\hat{n}}
\newcommand{\ho}{\hat{o}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hr}{\hat{r}}
\newcommand{\hs}{\hat{s}}
%\newcommand{\ht}{\hat{t}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}

\newcommand{\ta}{\tilde{a}}
\newcommand{\tb}{\tilde{b}}
\newcommand{\tc}{\tilde{c}}
\newcommand{\td}{\tilde{d}}
\newcommand{\te}{\tilde{e}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tg}{\tilde{g}}
%\newcommand{\th}{\tilde{h}}
\newcommand{\ti}{\tilde{i}}
\newcommand{\tj}{\tilde{j}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tl}{\tilde{l}}
\newcommand{\tm}{\tilde{m}}
\newcommand{\tn}{\tilde{n}}
%\newcommand{\to}{\tilde{o}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tq}{\tilde{q}}
\newcommand{\tr}{\tilde{r}}
\newcommand{\ts}{\tilde{s}}
%\newcommand{\tt}{\tilde{t}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tz}{\tilde{z}}

\newcommand{\tilt}{\tilde{t}}


\newcommand{\tA}{\tilde{A}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tI}{\tilde{I}}
\newcommand{\tJ}{\tilde{J}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tM}{\tilde{M}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tR}{\tilde{R}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tZ}{\tilde{Z}}


\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hI}{\hat{I}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hS}{\hat{S}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hW}{\hat{W}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hZ}{\hat{Z}}

\newcommand{\whA}{\widehat{A}}
\newcommand{\whB}{\widehat{B}}
\newcommand{\whC}{\widehat{C}}
\newcommand{\whD}{\widehat{D}}
\newcommand{\whE}{\widehat{E}}
\newcommand{\whF}{\widehat{F}}
\newcommand{\whG}{\widehat{G}}
\newcommand{\whH}{\widehat{H}}
\newcommand{\whI}{\widehat{I}}
\newcommand{\whJ}{\widehat{J}}
\newcommand{\whK}{\widehat{K}}
\newcommand{\whL}{\widehat{L}}
\newcommand{\whM}{\widehat{M}}
\newcommand{\whN}{\widehat{N}}
\newcommand{\whO}{\widehat{O}}
\newcommand{\whP}{\widehat{P}}
\newcommand{\whQ}{\widehat{Q}}
\newcommand{\whR}{\widehat{R}}
\newcommand{\whS}{\widehat{S}}
\newcommand{\whT}{\widehat{T}}
\newcommand{\whU}{\widehat{U}}
\newcommand{\whV}{\widehat{V}}
\newcommand{\whW}{\widehat{W}}
\newcommand{\whX}{\widehat{X}}
\newcommand{\whY}{\widehat{Y}}
\newcommand{\whZ}{\widehat{Z}}


\newcommand{\wha}{\widehat{a}}
\newcommand{\whb}{\widehat{b}}
\newcommand{\whc}{\widehat{c}}
\newcommand{\whd}{\widehat{d}}
\newcommand{\whe}{\widehat{e}}
\newcommand{\whf}{\widehat{f}}
\newcommand{\whg}{\widehat{g}}
\newcommand{\whh}{\widehat{h}}
\newcommand{\whi}{\widehat{i}}
\newcommand{\whj}{\widehat{j}}
\newcommand{\whk}{\widehat{k}}
\newcommand{\whl}{\widehat{l}}
\newcommand{\whm}{\widehat{m}}
\newcommand{\whn}{\widehat{n}}
\newcommand{\who}{\widehat{o}}
\newcommand{\whp}{\widehat{p}}
\newcommand{\whq}{\widehat{q}}
\newcommand{\whr}{\widehat{r}}
\newcommand{\whs}{\widehat{s}}
\newcommand{\wht}{\widehat{t}}
\newcommand{\whu}{\widehat{u}}
\newcommand{\whv}{\widehat{v}}
\newcommand{\whw}{\widehat{w}}
\newcommand{\whx}{\widehat{x}}
\newcommand{\why}{\widehat{y}}
\newcommand{\whz}{\widehat{z}}


\newcommand{\olh}{\overline{h}}
\newcommand{\ulh}{\underline{h}}

\newcommand{\oA}{\overline{A}}
\newcommand{\oB}{\overline{B}}
\newcommand{\oC}{\overline{C}}
\newcommand{\oD}{\overline{D}}
\newcommand{\oE}{\overline{E}}
\newcommand{\oF}{\overline{F}}
\newcommand{\oG}{\overline{G}}
\newcommand{\oH}{\overline{H}}
\newcommand{\oI}{\overline{I}}
\newcommand{\oJ}{\overline{J}}
\newcommand{\oK}{\overline{K}}
\newcommand{\oL}{\overline{L}}
\newcommand{\oM}{\overline{M}}
\newcommand{\oN}{\overline{N}}
\newcommand{\oO}{\overline{O}}
\newcommand{\oP}{\overline{P}}
\newcommand{\oQ}{\overline{Q}}
\newcommand{\oR}{\overline{R}}
\newcommand{\oS}{\overline{S}}
\newcommand{\oT}{\overline{T}}
\newcommand{\oU}{\overline{U}}
\newcommand{\oV}{\overline{V}}
\newcommand{\oW}{\overline{W}}
\newcommand{\oX}{\overline{X}}
\newcommand{\oY}{\overline{Y}}
\newcommand{\oZ}{\overline{Z}}

\newcommand{\pB}{B^+}
\newcommand{\mB}{B^-}
\newcommand{\pD}{D^+}
\newcommand{\mD}{D^-}
\newcommand{\pJ}{J^+}
\newcommand{\mJ}{J^-}


\newcommand{\dif}{\mathrm{d}\:\!}
%\newcommand{\dif}{\mathrm{d}\,}
\newcommand{\Dif}{\mathrm{D}}
\newcommand{\Leb}{\mathrm{Leb}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\grad}{\mathrm{grad}}

\newcommand{\inprod}[2]{\langle{#1},{#2}\rangle}


\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}


%\DeclareMathOperator{\dif}{\mathrm{d}}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\diam}{diam} %diameter
\DeclareMathOperator{\dist}{dist} %distance
\DeclareMathOperator{\dom}{dom} %domain of a map
\DeclareMathOperator{\cl}{cl} %closure of a set
\DeclareMathOperator{\inr}{int} %interior of a set
\DeclareMathOperator{\Comp}{Comp} %connected component in complex plane
\DeclareMathOperator{\comp}{comp} %connected component in real line
\DeclareMathOperator{\suchthat}{s.t.} %connected component

%\newcommand{\textif}{\text{if }}
%\newcommand{\textthen}{\text{then }}
\newcommand{\textfor}{\quad\text{for}\quad}
\newcommand{\textand}{\quad\text{and}\quad}
\newcommand{\textandd}{\qquad\text{and}\qquad}

\newcommand{\qtext}[1]{\quad\text{#1}\quad}

